XMem: Long-Term Video Object Segmentation with an Atkinson-Shiffrin Memory Model

We present XMem, a video object segmentation architecture for long videos with unified feature memory stores inspired by the Atkinson-Shiffrin memory model. Prior work on video object segmentation typically only uses one type of feature memory. For videos longer than a minute, a single feature memory model tightly links memory consumption and accuracy. In contrast, following the Atkinson-Shiffrin model, we develop an architecture that incorporates multiple independent yet deeply-connected feature memory stores: a rapidly updated sensory memory, a high-resolution working memory, and a compact thus sustained long-term memory. Crucially, we develop a memory potentiation algorithm that routinely consolidates actively used working memory elements into the long-term memory, which avoids memory explosion and minimizes performance decay for long-term prediction. Combined with a new memory reading mechanism, XMem greatly exceeds state-of-the-art performance on long-video datasets while being on par with state-of-the-art methods (that do not work on long videos) on short-video datasets. Code is available at https://hkchengrex.github.io/XMem

==> results/lt-vis.tex <==
\begin{tabular}{c@{\hspace{1mm}}c@{\hspace{.5mm}}c@{\hspace{.5mm}}c@{\hspace{.5mm}}c@{\hspace{.5mm}}c}
	\rotatebox[origin=c]{90}{\scriptsize Images \hspace{1mm}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/00000.jpg}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/02256.jpg}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/03588.jpg}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/04168.jpg}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/10748.jpg}}\\
	\vspace{-2.5mm}&&&&&\\
	\rotatebox[origin=c]{90}{\scriptsize JOINT \hspace{1mm}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/00000.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/jo_02256.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/jo_03588.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/jo_04168.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/jo_10748.png}}\\
	\vspace{-2.5mm}&&&&&\\
	\rotatebox[origin=c]{90}{\scriptsize AFB-URR \hspace{1mm}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/00000.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/af_02256.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/af_03588.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/af_04168.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/af_10748.png}}\\
	\vspace{-2.5mm}&&&&&\\
	\rotatebox[origin=c]{90}{\scriptsize STCN \hspace{1mm}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/00000.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/st_02256.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/st_03588.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/st_04168.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/st_10748.png}}\\
	\vspace{-2.5mm}&&&&&\\
	\rotatebox[origin=c]{90}{\scriptsize Ours \hspace{1mm}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/00000.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/ours_02256.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/ours_03588.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/ours_04168.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/ours_10748.png}}\\
	\vspace{-2.5mm}&&&&&\\
	\rotatebox[origin=c]{90}{\scriptsize GT \hspace{1mm}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/00000.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/02256.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/03588.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/04168.png}}&
	\raisebox{-0.5\height}{\includegraphics[width=0.18\linewidth]{results/10748.png}}\\
	\vspace{-2mm}&&&&&\\
	& Frame 0 (input) & Frame 2256 & Frame 3588 & Frame 4168 & Frame 10748 \\
\end{tabular}
